Question-Aware Knowledge Graph Prompting for Enhancing Large Language Models

Large Language Models (LLMs) often struggle with tasks requiring external knowledge, such as knowledge-intensive Multiple Choice Question Answering (MCQA). Integrating Knowledge Graphs (KGs) can enhance reasoning; however, existing methods typically demand costly fine-tuning or retrieve noisy KG information. Recent approaches leverage Graph Neural Networks (GNNs) to generate KG-based input embedding prefixes as soft prompts for LLMs but fail to account for question relevance, resulting in noisy prompts. Moreover, in MCQA tasks, the absence of relevant KG knowledge for certain answer options remains a significant challenge. To address these issues, we propose Question-Aware Knowledge Graph Prompting (QAP), which incorporates question embeddings into GNN aggregation to dynamically assess KG relevance. QAP employs global attention to capture inter-option relationships, enriching soft prompts with inferred knowledge. Experimental results demonstrate that QAP outperforms state-of-the-art methods across multiple datasets, highlighting its effectiveness.

==> table.tex <==
\begin{table*}[t]\centering
\caption{\label{result}
Comparison between the accuracy(\%) and standard deviation(\%) over QAP and baselines on the tasks on the three datasets. %$\sigma$ is the standard variance. 
The best and second-best results are respectively shown in \textbf{bold} and \underline{underlined}.
}
\renewcommand{\arraystretch}{1.6}
\setlength\tabcolsep{5.6pt}

%\scalebox{1.1}{
\begin{tabular}{c|ccc|ccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Method}}& \multicolumn{3}{c|}{Flan-T5 (3B)} & \multicolumn{3}{c}{Flan-T5 (11B)} \\  \cline{2-7}
& OBQA      & Riddle   & MedQA% &Mean%&$\sigma$ 
& OBQA     & Riddle    & MedQA% &Mean %&$\sigma$
\\ \hline
LLM &
  73.60\pm0.10 &
  55.29\pm0.20 &
  34.25\pm0.04 &
  % 54.38 %&19.69   
  % &
  80.40\pm0.10 &
  66.08\pm 0.10&
  39.28\pm0.08% &61.92%&20.87
  \\
PE         & 75.00\pm 0.50  & 55.88\pm 0.49   & \underline{34.49}\pm 0.20 %&55.12%&20.27 
& 83.20\pm  0.30  & 65.29\pm   0.20  & 39.67\pm 0.24% &  61.92%&21.88
\\
KGEP & 73.00\pm  0.60 & 48.43\pm 1.18   & 30.56\pm 0.47% &50.66%&21.31 
& 78.00\pm  1.00  & 61.37\pm  1.18   & 34.41\pm 0.50%5  & 57.93 %&22.00
\\
SP                & 75.60\pm 0.40  & 54.31\pm 0.59   & 34.33\pm 0.31 %& 54.75%& 20.64
& 84.60\pm  0.20  & 65.29\pm  1.57   & 39.28\pm 0.08  %& 63.06%&22.74
\\
GNP         & \underline{76.20}\pm 0.80  & \underline{57.06}\pm 0.98  & 34.01\pm 0.55  %& 55.76 %&21.13
& \underline{85.40}\pm 0.80   & \underline{67.84}\pm  0.78   & \underline{39.91}\pm 0.63  %& 64.38%&22.94
\\
\cellcolor{gray!21}{QAP  }                 & \cellcolor{gray!21}{\textbf{82.00}}\pm 0.50  & \cellcolor{gray!21}{\textbf{68.82}}\pm 0.20   & \cellcolor{gray!21}{\textbf{38.57}}\pm 1.02  %&\cellcolor{gray!21}{\textbf{63.13}}         %&\cellcolor{gray!21}{22.27}
   &
\cellcolor{gray!21}{\textbf{88.20}}\pm  0.60  & \cellcolor{gray!21}{\textbf{77.06}}\pm   0.39  & \cellcolor{gray!21}{\textbf{44.30}}\pm0.47 %&\cellcolor{gray!21}{\textbf{69.85}}%&\cellcolor{gray!21}{22.82}
\\\hline
\end{tabular}
\vspace{-10pt}
\end{table*}






















\begin{table*}[!t]\centering
\caption{\label{ablation}
Experimental results of ablation studies. This table present the accuracy(\%) of the studies and standard deviation(\%) on the three datasets. The best results are shown in \textbf{bold}, respectively. Here ``w/o QNA", ``w/o IPT" and ``w/o MH" respectively represent the removal of QNA, IPT and multiple heads.
}
\renewcommand{\arraystretch}{1.5}
\setlength\tabcolsep{3.1pt}

% \scalebox{0.9}{
\begin{tabular}{c|ccc|ccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Method}}& \multicolumn{3}{c|}{Flan-T5 (3B)} & \multicolumn{3}{c}{Flan-T5 (11B)} \\  \cline{2-7}
& OBQA      & Riddle   & MedQA %& Decline 
& OBQA     & Riddle    & MedQA %&Decline   
\\ \hline
\cellcolor{gray!21}{QAP}                 & \cellcolor{gray!21}{\textbf{82.00}}\pm0.50  & \cellcolor{gray!21}{\textbf{68.82}}\pm0.20  & \cellcolor{gray!21}{\textbf{38.57}}\pm1.02 & 
  % \cellcolor{gray!21}{\textbf{-}}        
   
\cellcolor{gray!21}{\textbf{88.20}}\pm0.60  & \cellcolor{gray!21}{\textbf{77.06}}\pm0.39 & \cellcolor{gray!21}{\textbf{44.30}}\pm 0.47%&\cellcolor{gray!21}{\textbf{-}}
\\
QAP w/o QNA &
   75.60\pm1.00&
   63.53\pm0.20&
    34.87\pm1.18&
      
   84.40\pm1.10&
   68.04\pm0.29&
   42.26\pm0.31%&6.87
  \\
QAP w/o IPT &
   76.60\pm0.90&
   63.73\pm0.29&
   35.19\pm1.26&
      
   82.40\pm0.80&
   66.67\pm0.39&
   42.73\pm0.55%&7.87
  \\
QAP w/o MH &
   76.40\pm1.20&
   63.92\pm0.39&
   35.42\pm0.86&
       
   85.00\pm1.40&
   70.39\pm0.59&
   43.05\pm0.24%&5.04
  \\



\hline

\end{tabular}
\vspace{-7pt}
\end{table*}

